Context-Aware Interaction Network for Question Matching

Impressive milestones have been achieved in text matching by adopting a cross-attention mechanism to capture pertinent semantic connections between two sentence representations. However, regular cross-attention focuses on word-level links between the two input sequences, neglecting the importance of contextual information. We propose a context-aware interaction network (COIN) to properly align two sequences and infer their semantic relationship. Specifically, each interaction block includes (1) a context-aware cross-attention mechanism to effectively integrate contextual information when aligning two sequences, and (2) a gate fusion layer to flexibly interpolate aligned representations. We apply multiple stacked interaction blocks to produce alignments at different levels and gradually refine the attention results. Experiments on two question matching datasets and detailed analyses demonstrate the effectiveness of our model.

==> EMNLP 2021 COIN-camera-ready/abstract.tex <==
Impressive milestones have been achieved in text matching by adopting a cross-attention mechanism to capture pertinent semantic connections between two sentence representations.
However, regular cross-attention focuses on word-level links between the two input sequences, neglecting the importance of contextual information.
We propose a context-aware interaction network (COIN) to properly align two sequences and infer their semantic relationship.
Specifically, each interaction block includes (1) a context-aware cross-attention mechanism to effectively integrate contextual information when aligning two sequences, and (2) a gate fusion layer to flexibly interpolate aligned representations.
We apply multiple stacked interaction blocks to produce alignments at different levels and gradually refine the attention results. 
Experiments on two question matching datasets and detailed analyses demonstrate the effectiveness of our model.


==> EMNLP 2021 COIN-camera-ready/analysis.tex <==

\subsection{Model Analysis}\label{ablation}

\begin{table}[t]
\fontsize{9}{11}\selectfont
\vspace{-2mm}
 \setlength{\tabcolsep}{1.2mm}
  \centering
    \begin{tabular}{|l|cc|}
        \hline
        Model & Quora & LCQMC \\
         \hline
        original & 89.6 & 85.4   \\
        w/o context & 89.1 & 84.8  \\
        simple fusion & 88.8 & 85.2 \\
        w/o aggregat. & 89.2 & 84.9  \\
        simple pool & 89.4  & 85.2  \\
        \hline
    \end{tabular}
    \vspace{2mm}
    \caption{
    Ablation study on Quora and LCQMC dev set.
    } 
    \label{tab:ablation}
    \vspace{-2mm}
\end{table}


\smallskip
\noindent\textbf{Effect of Model Components.} 
In Table~\ref{tab:ablation}, we study the contribution of different model components. Without context in cross-attention, the accuracy decreases by 0.5 and 0.6 percentage points, respectively. This confirms that, by incorporating the context, our model can better capture sentence relationships in the alignments. We then replace the gate fusion with a simplified fusion layer, where we feed the concatenation of the two representations to a feed-forward network, observing a performance drop on both datasets. This shows the effectiveness of our context-aware interaction blocks.
We then remove the aggregation layer, finding that the accuracy decreases to $89.2\%$ and $84.9\%$. This confirms that the aggregation layer is useful to produce high-level representations for the final prediction. In the last ablation, we replace the multi-head pooling by max-pooling to produce the sentence vector, and the results decrease on both datasets.


\begin{figure}[t]
    \centering
    \vspace{-2mm}
    \includegraphics[scale=0.53]{fig/interaction_num_ablation.pdf}
    \vspace{-3mm}
    \captionof{figure}{ 
     Ablation study [Left] and effect of number of interaction blocks [Right] on Quora and LCQMC dev sets.
    }
    \label{fig:interaction_num_ablation}
    \vspace{-2mm}
\end{figure} 

\smallskip
\noindent\textbf{Effect of Interaction Block Depth.}
Figure~\ref{fig:interaction_num_ablation} plots the accuracy with varying numbers of interaction blocks. Evidently, a smaller number of interaction blocks may not suffice to fully capture the sentence relationships, and adding further such blocks may improve the model's ability to reason across the sequences and boost the performance. However, increasing the depth of interactions more than necessary harms the performance. Additionally, there is a trade-off between performance and efficiency since adding more interaction blocks increases the number of  parameters. For computational cost reasons, we use at most three interactions blocks in our experiments.

\smallskip
\noindent\textbf{Case Study.}

We analyze the context-aware interaction results by visualizing the attention to show how the model learns aligned features at different levels of interaction in Figure~\ref{fig:att-visual}. We consider a sample from Quora with the target label \textsc{Duplicate}.

The left image shows the contextualized cross-attention in the first interaction block. Aided by the context, the model learns to correctly align the salient phrase ``\textit{new macbook pro}" across the inputs. 
The attention results in the third interaction block are visualized in the right image. As we can observe, the model refines the alignment results with a sharper distribution on the salient phrases than in the first interaction block, and the structured phrase ``\textit{what do you think of}" is also connected.  
The model thus predicts the relationship between the two sentences correctly. This corroborates our model's ability to gradually refine and adjust the attention scores in higher layers.

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.32]{fig/attention_coin.pdf}
    \vspace{-7mm}
    \captionof{figure}{ 
    Visualization of alignment in the first and third interactions. Lighter colors indicate higher values.
    }
    \label{fig:att-visual}
    \vspace{-4mm}
\end{figure}






==> EMNLP 2021 COIN-camera-ready/conclusion.tex <==
In this work, we propose a context-aware interaction network for question matching. We improve the cross-attention by incorporating contextual cues, and further leverage a gate fusion layer to flexibly integrate the aligned features. 
Experiments on two datasets validate the effectiveness of our architecture and show that accounting for the context enhances the original cross-attention.


==> EMNLP 2021 COIN-camera-ready/experiments.tex <==


\subsection{Experimental Setup}
\noindent\textbf{Datasets.} 
We conduct experiments on two datasets: 1) The Quora Questions Pairs corpus (Quora) contains over 400k English question pairs selected from Quora.com, for which we use the same data split as \newcite{wang2017bilateral}. 2) LCQMC~\cite{liu-etal-2018-lcqmc} is a large-scale open-domain Chinese question matching corpus constructed from Baidu Knows. We follow the data splits in the original papers, and apply a hard cut-off of the sentence length on both datasets by cropping or padding. The length is set to 32 for Quora and 50 for LCQMC.



\smallskip
\noindent\textbf{Training Details and Parameters.} 
For Quora, we use 300 dimensional GloVe embeddings~\cite{pennington-etal-2014-glove}.
For LCQMC, following \newcite{li-etal-2019-word-segmentation}, we avoid word segmentation and instead use a randomly initialized character embedding matrix. The kernel size is 3 for convolutional layers with padding. We tune the dimensionality of the feed-forward layers from 150 to 300. The batch size is tuned from 32 to 128. Adam optimization is used with an initial learning rate of 0.001 and exponential decay. We 
use ReLU~\cite{pmlr-v15-glorot11a} as the activation function in all feed-forward networks. To prevent over-fitting, dropout with a retention probability of 0.8 is applied. We apply 3 context-aware interaction blocks for Quora and 2 interaction blocks for LCQMC. For BERT~\cite{devlin-etal-2019-bert}, we choose the BERT-base version (12 layers, 768 hidden dimensions and 12 attention heads). Further training details are given in the appendix.


\begin{table}[t]
\fontsize{8}{10}\selectfont
 \setlength{\tabcolsep}{1.56mm}
  \centering
    \begin{tabular}{|l|c|c|}
        \hline
        {\bf Model} & {\bf  Acc (\%)} & {\bf F1 (\%)} \\
        \hline
        
        Lattice-CNN & 82.1 & 82.4 \\
        ESIM~\cite{chen-etal-2017-enhanced} & 82.0 & 84.0 \\
        BiMPM~\cite{wang2017bilateral} & 83.3 & 84.9 \\
        GMN~\cite{chen-etal-2020-neural-graph} & 84.6 & 86.0 \\
        COIN (Ours)  &  {\bf85.6}& {\bf 86.5} \\
        \hline
        BERT~\cite{devlin-etal-2019-bert} & 85.7 & 86.8 \\
        SBERT~\cite{reimers-gurevych-2019-sentence} & 85.4 & 86.6 \\
         COIN (ensemble)  &  {\bf86.2} & {\bf 87.0} \\
        \hline
    \end{tabular}
    \vspace{2mm}
    \caption{
    Experimental results on LCQMC.
    }
    \label{tab:lcqmc-result}
    \vspace{-4mm}
\end{table}

\begin{table}[t]
\fontsize{8}{10}\selectfont
 \setlength{\tabcolsep}{1.56mm}
  \centering
    \begin{tabular}{|l|c|r|}
        \hline
        {\bf Model} & {\bf Acc. (\%)} & {\bf Params}\\
        \hline
        BiMPM~\cite{wang2017bilateral} & 88.2 & 1.6M \\
        DIIN~\cite{gong2017natural} & 89.0 & 4.4M \\
        CAFE~\cite{tay-etal-2018-compare} & 88.7 & 4.7M \\
        OSOA-DFN~\cite{liu-etal-2019-original} & 89.0 & 10.0M \\
        RE2~\cite{yang-etal-2019-simple} & 89.2 & 2.8M \\
        ESAN~\cite{hu-etal-2020-enhanced} & 89.3 & 3.9M \\
        Enhanced-RCNN~\cite{peng2020enhanced} & 89.3 & 7.7M \\
        COIN (ours) &  {\bf89.4} & 6.5M   \\
        \hline
         BERT~\cite{devlin-etal-2019-bert} & 90.1 & 109.5M  \\
         SBERT~\cite{reimers-gurevych-2019-sentence} & 90.6 & 109.5M \\
         COIN (ensemble) &  {\bf90.7} & 32.5M \\
        \hline
    \end{tabular}
    \vspace{2mm}
    \caption{
    Experimental results on Quora dataset. 
    }
    \label{tab:quora-result}
    \vspace{-4mm}
\end{table}


\subsection{Experimental Results}\label{results}
We compare our model against recent prior work, including state-of-the-art neural models and BERT based methods. ESIM~\cite{chen-etal-2017-enhanced} and BiMPM~\cite{wang2017bilateral} are two strong sentence-interaction baselines. GMN~\cite{chen-etal-2020-neural-graph} is a neural graph matching network with multi-granular input information. DIIN~\cite{gong2017natural} extracts semantic features from the interaction space.
OSOA-DFN~\cite{liu-etal-2019-original} uses multiple original semantics-oriented attention, and
RE2~\cite{yang-etal-2019-simple} adopts richer features for alignment processes to improve the performance. ESAN~\cite{hu-etal-2020-enhanced} is a sentence-interaction model with gated feature augmentation. For pre-trained methods, we consider BERT~\cite{devlin-etal-2019-bert} and SBERT~\cite{reimers-gurevych-2019-sentence}. We also include ensemble results of our method where we consider the majority vote of the results given by 5 runs of the same model under different random parameter initialization.

Results on LCQMC are listed in Table~\ref{tab:lcqmc-result}. Our single model achieves better accuracy and F1-score than all non-pretrained baselines, and the results of COIN are fairly comparable to BERT despite \emph{not} being pretrained on any extrinsic data. In fact, our ensemble model (5 runs) even outperforms BERT.

The results on Quora are given in Table~\ref{tab:quora-result}. Our approach outperforms the non-pretrained baselines with 89.4\% test accuracy, and our ensemble model again achieves better results than BERT and SBERT with fewer parameters (32.5M vs.\ 109.5M). This confirms our model's ability to be applied in real-world scenarios that require less computational complexity and a smaller model footprint.

Overall, the above results on two question matching datasets reflect our model's effectiveness at capturing semantic interactions between the sentences and properly interring their relationship. In-depth analyses of the model's efficiency are given in the appendix.





\input{analysis}




==> EMNLP 2021 COIN-camera-ready/fig/intro.tex <==
Natural language inference, which is also known as recognizing textual entailment (RTE), is a fundamental task in natural language processing. Given a premise sentence and a hypothesis sentence, the model needs to predict whether the premise can infer the hypothesis~\cite{bowman-etal-2015-large}. 
This is a challenging task because it requires model to deeply understand the texts, capture proper language patterns, and conduct correct logical reasoning in different levels which also relies on commonsense knowledge~\cite{storks2019recent}. 
% \yucomment{change to: it requires model to capture language patterns and text relatedness in different levels (\ie word-, and sentence- level)?}

% \begin{figure}[t]
%     \def\arraystretch{1.1}
%     \bgroup
%     % \def\arraystretch{1.1}
% 	\fontsize{9}{10}\selectfont
%      \hspace{-1mm}
% 	\setlength{\tabcolsep}{0.8mm}
% 	\begin{tabular}{|p{75mm}|}
% 	\hline
% % 	\vspace{0.03mm}
% 	\textbf{Premise}: A group of kids is splashing in deep water nearby a rock formation. \\
% 	\textbf{Hypothesis}: The kids are in deep water. \\
% 	\textbf{Label}: \textit{Entailment} \\
% 	\\
% 	\textbf{Premise}: A busy street with numerous people interacting and going about their lives. \\
% 	\textbf{Hypothesis}: The morning rush hour fills the streets with busy people. \\
% 	\textbf{Label}: \textit{Neutral} \\ 
% 	\vspace{0.3mm}
% 	\textbf{Premise}: The little boy gets ready to kick the soccer ball. \\
% 	\textbf{Hypothesis}: The boy is sleeping at home. \\
% 	\textbf{Label}: \textit{Contradiction} \\
	
% 	\hline
% % 	\vspace{0.03mm}
% 	\textbf{Text1}: What should I do to avoid sleeping in class? \\
% 	\textbf{Text2}: How do I not sleep in a boring class? \\
% 	\textbf{Label}: \textit{Paraphrase} \\
% 	\\
% 	\textbf{Text1}: What is the best time to read MBA? \\
% 	\textbf{Text2}: What 's the best time for reading? \\
% 	\textbf{Label}: \textit{Non-paraphrase} \\
%     \hline
	
% 	\end{tabular}
%     \vspace{-3mm}
% \caption{Examples for natural language inference and paraphrase identification. The samples in the upper box are taken from SNLI dataset, and in the bottom box are from Quora dataset.} 
% \label{fig:sample-keyphrase}
% \egroup
% \vspace{-5mm}
% \end{figure}


% \begin{figure*}[t]
%     \centering
%     \includegraphics[scale=0.6]{fig/model_figure2.pdf}
%     \captionof{figure}{ 
%     Our proposed model structure. On the left is the main framework of SENAN, which has 4 parts: a representation layer, multiple stacked interactions blocks, a aggregation layer and a final prediction layer. On the right is detailed structure of the self-aware interaction block consisting of a two-hop attention and a gate fusion operation.
%     \todo{modify the figure color}
%     }
%     \label{fig:model_structure}
%     % \vspace{-4mm}
% \end{figure*}

Recently neural network approaches have been successfully applied to NLI with the availability of large-scale annotated datasets and the development of deep learning techniques~\cite{bowman-etal-2015-large,williams-etal-2018-broad,chen-etal-2017-enhanced,wang2017bilateral,wang-jiang-2016-learning}. Most existing neural models fall into two types, namely sentence encoding approach and sentence interaction approach. The former encodes sentences into vector representations and makes the prediction based on them, while the latter considers interactions between two sequences to capture their semantic relations and usually achieves better results.


Attention mechanism has been widely adopted in sentence interaction approach where a word-by-word attention matrix is computed to get aligned information between two sequences. This method has been proved to be useful to address NLI task~\cite{gong2017natural,parikh-etal-2016-decomposable,rocktaschel2015reasoning,wang-jiang-2016-learning}.
% \yucomment{change to: This method has proved useful to address the text matching task.}
Nevertheless, when computing the word-level cross sentence attention, existing models only focus on local matching and insufficiently consider global semantics: each element of the attention matrix is calculated by two individual tokens from the sequences without direct consideration of the global contexts. 
% \yucomment{It's not clear what are you trying to say in the rest of this paragraph. Is this a second motivation? Or is it the solution you proposed?} 

When human conduct this task, they tend to first go through each sentence and pay attention to the salient contents (similar as conducting self-attention on each sequence), and then compare against the other sentence and connect the relevant elements such as words or phrases to learn their relations (can be viewed as cross-attention between two sequences). Usually this procedure is conducted for multiple times to get a better understanding of the sentence relationship, and then make the final prediction.

Inspired by this, we propose a 
\underline{SE}lf-aware I\underline{N}ter\underline{A}ction \underline{N}etwork
(SENAN) with a novel self-aware interaction block to capture sequence relations and update the sentence representations, as shown in Figure~\ref{fig:model_structure}. Concretely, the self-aware interaction block consists of a two-hop attention and a gate fusion layer. 
In two-hop attention, the model first computes self-alignment attention for each sequence to enrich the original representations with salient contextual features, and then conducts a cross sentence attention to produce proper alignments for semantic reasoning.
The gate fusion layer is designed to enable model to selectively integrate the aligned representations and control how much the new information to be passed to the following layers. 
In addition, We apply stacked interaction blocks to strength the model ability on refining the attention distributions and updating sentence representations progressively. This forms a 
\textbf{multi-step reasoning process}. We then adopt an aggregation layer to produce high-level semantic representations for the premise and hypothesis, and predict the result based on the refined representations. 

To validate the effectiveness of our proposed method, we conduct extensive experiments on SNLI, MultiNLI, SciTail and Quora Questions Pairs datasets, and provide analysis on model components and a case study through visualization of alignment results\footnote{We will release our code upon publication.}. The overall contributions of our work can be summarized as follows:
\begin{itemize}
% \smallskip
\item We propose a novel self-aware interaction network with a two-hop attention to produce proper alignments between two sequences. The multiple interactions are applied to let model gradually learn semantic relatedness and refine attention results.

\item We design a gate fusion layer to flexibly integrate the aligned features and update sequence representations from different levels. 
% The gate mechanism can be also viewed as a shortcut connection to reduce the training difficulty. 
An aggregation layer is applied to produce high-level semantic representations of each sentences for prediction.

\item We evaluate our model capacity on four benchmark NLI (alike)  datasets with extensive experiments. Our approach outperforms strong comparisons with competitive results, which validates the model effectiveness for solving natural language inference task.

% \item We propose a two-hop attention operation which consists of a self-attention and a cross-attention, to capture proper alignments of two sequences. We apply multiple interactions to learn different levels of relatedness and gradually refine the alignment results.

% \item We design a gate fusion to flexibly integrate aligned features and update sequence representations from different levels. An aggregation layer is applied to produce final sequence representations for the prediction.

% \item We evaluate our model capacity on four benchmark datasets, and the results show our approach outperforms strong comparisons with competitive results.
\end{itemize}


==> EMNLP 2021 COIN-camera-ready/fig/model.tex <==
% \section{Our Model}
\begin{figure*}[t]
    \centering
    % \includegraphics[scale=0.63]{fig/model_figure5.pdf}
    \includegraphics[scale=0.63]{fig/model-yy.pdf}
    \captionof{figure}{ 
    Our proposed model structure. On the left is the main framework of SENAN, which has 4 parts: a representation layer, stacked interactions blocks, an aggregation layer and a final prediction layer. On the right is detailed structure of the self-aware interaction block consisting of a two-hop attention and a gate fusion layer.
    }
    \label{fig:model_structure}
    \vspace{-5mm}
\end{figure*}

Natural language inference can be viewed as a classification task that predicts the label $Y$ for a given premise-hypothesis pair $(S_a, S_b)$, where $Y$ = \{\textit{entailment}, \textit{contradiction}, \textit{neutral}\}. We propose an interaction based neural approach to tackle this problem as shown in Figure~\ref{fig:model_structure}. 


% Unlike existing models for this task, our model: (1) Consists of self-aware interactions blocks which combines self-attention and inter-sentences alignment; (2) Fuses sentence information and alignment information by a gated fusion layer to let the model flexibly control the information pass to the next layer' (3) Utilizes an aggregation layer after interaction blocks to get the final representation. 

% In our model, each sentence is embedded on both char-level and word-level. The concatenation of both embeddings is then used as input for the encoder, a simple CNN encoder. In order to keep more information before passing through the encoder, instead of only the encoding, the concatenation of embeddings and encoding is fed to a self-aware attentive alignment module. The module is composed of N blocks with identical structures and independent parameters. Each block: (1) is not only consisted of inter-sentence alignment, but also of self-attention of each sentence; (2) uses gated fusion mechanism to incorporate alignments into sentence representations. Details of the alignment module will be discussed below in section **. After the module, alignment representations for each sentence are then aggregated, pooled and fed to classification layer. Except for the alignment layer, symmetric architectures are used for both input sentences, using shared the parameters.

In our approach, each sentence is first embedded and encoded to get the sentence representations. Then we design a self-aware interaction block to properly align two sequences and capture their semantic relatedness for the logical reasoning.
% which consists of (1) a two-hop attention operation with both self-attention and cross-attention,
% and (2) a gate fusion layer to flexibly integrate aligned information.
% , which lets the model flexibly control how much information to be passed to the next layer. 
In addition, we apply multiple interaction blocks with independent parameters to gradually learn semantic relations and reason between two sequences in different levels. Details of the self-aware interaction block will be discussed below in Section \ref{Self-aware Interaction Block}. Then the representations for each sentence are aggregated, pooled and fed to a classification layer. Symmetric architecture is used for both input sentences with shared parameters.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[scale=0.6]{fig/model_figure2.pdf}
%     \captionof{figure}{ 
%     Our proposed model structure. On the left is the main framework of SENAN, which has 4 parts: a representation layer, multiple stacked interactions blocks, a aggregation layer and a final prediction layer. On the right is detailed structure of the self-aware interaction block consisting of a two-hop attention and a gate fusion operation.
%     \todo{modify the figure color}
%     }
%     \label{fig:model_structure}
%     % \vspace{-4mm}
% \end{figure*}

\subsection{Input Representation Layer}

% The encoding layer first converts sentence pairs into embeddings. In our model, both character embeddings and word embeddings are used. Given a sentence pair $Q=[q_w_1, ..., q_w_i, ..., q_w_m]$, $P=[p_w_1, ..., p_w_j, ..., p_w_n]$, where $q_w_i$ and $p_w_j$ denotes the $i$-th and $j$-th word of $Q$ and $P$ respectively, a pre-trained look-up table $M_w$ is leveraged to convert $Q$ and $P$ into vectors. $Q$ and $P$

The input representation layer converts each sentence into matrix representations with an embedding and encoding layer. 

\smallskip
\noindent \textbf{Embedding.} 
In our model, both word embeddings and character embeddings are used. To get the character-based word representations, we apply a convolutional neural network (CNN) with max pooling over the entire tokens ~\cite{kim2016character}. The character embeddings have been shown to be useful for out-of-vocabulary (OOV) problem. For word embeddings, we adopt the commonly used Glove embeddings~\cite{pennington-etal-2014-glove} to represent each token as a vector. Following \newcite{seo2016bidirectional}, the outputs of word embeddings and character embeddings are concatenated, and then passed through a 2-layer highway network~\cite{srivastava2015highway} to get the final representation of each single word. 

\smallskip
\noindent \textbf{Encoding.} To encode the contextual information into token representations, we use a stacked Bidirectional LSTM (Bi-LSTM)~\cite{hochreiter1997long} encoder on the top of the embedding layer to model temporal interactions between words,
% Following \newcite{tay-etal-2018-co}, we apply a stacked recurrent encoder layer,
% Hence we obtain the contextual representations of two sentences
% % $\mathbf{H}_a=[\mathbf{h}_{a_1}, ..., \mathbf{h}_{a_i}, ..., \mathbf{h}_{a_m}]$ and $\mathbf{H}_b=[\mathbf{h}_{b_1}, ..., \mathbf{h}_{b_j}, ..., \mathbf{h}_{b_n}]$, where $\mathbf{H}_a \in \mathbb{R}^{m \times d}$ and $\mathbf{H}_b \in \mathbb{R}^{n \times d}$.
% $\mathbf{H}^0_a=\{\mathbf{h}^0_{a_i}|\mathbf{h}^0_{a_i} \in \mathbb{R}^{2d}, i=1,2,...,m \}$ and $\mathbf{H}^0_b=\{\mathbf{h}^0_{b_j}|\mathbf{h}^0_{b_j} \in \mathbb{R}^{2d}, i=1,2,...,n \}$, where d is the hidden dimension of the forward and backward LSTMs. 
and hence obtain the contextual representations. 
% Inspired by \newcite{yang-etal-2019-simple}, 
In addition, we concatenate the contextual representations with the original embedding vectors to produce better alignments in the following interaction blocks. This is similar as a skip connection to represent words in different levels~\cite{wang-etal-2018-multi}.



\subsection{Self-aware Interaction Block}\label{Self-aware Interaction Block}
% Recently the attention-based neural models have achieved good performance on text matching~\cite{rocktaschel2015reasoning,chen-etal-2017-enhanced,parikh-etal-2016-decomposable,duan2018attention}. 
Our proposed self-aware interaction block consists of
a two-hop attention and a gate fusion layer. The attention is responsible for aligning two sequences and capturing their semantic relationship. 
% We strength the cross-sentence attention to a two-hop style with a self-attention so that the model can better identify the salient contextual features. 
We strength the model with ability to better identify the salient contextual features and properly capture sequence alignments by extending the normal cross-sentence attention to a two-hop style, with an additional self-alignment attention. 
Then the gate fusion layer is leveraged to flexibility integrate the aligned features and update sequence representations.
% to properly capture the alignments between two sequences and selectively integrate the aligned features and update the sequence representations. 
% For the two-hop attention, the model first computes self-attention for each sequence to identify the salient contextual features, and then conducts cross-sentence attention to get aligned representations. 
% By doing this, the model is strengthened with the capacity to better reason between two sentences by capturing the relevant information with salient semantic features. 
% A gate fusion layer is adopted to flexibility fuse the aligned features and update sequence representations.
% \yucomment{change to: A gate fusion layer is adopted to control the amount of information being propagated to the following layers and hence increase the flexibility of the model.} 
In addition, inspired by the idea of end-to-end memory network~\cite{sukhbaatar2015end}, we apply multiple stacked interaction blocks so that our model can gradually refine the alignment results and integrate the inferential information from different levels.

\smallskip
\noindent \textbf{Two-hop Attention.} 
% We applied self-aware alignment to capture semantic features correlated to the relationship of two sentences. Specifically, self-attentive representation of each sentence and inter-alignment are computed. For simplification, we present below the computations on $\mathbf{H}^0_a$. We first concatenate the encoding $\mathbf{H}^0_a$ with its embedding(**Undefined symbol**). The concatenated vectors are then utilized as input for a self attentive representation $\tilde{H}^0_a \in \mathbb{R}^{2d \times 1}$, where $\tilde{H}^0_a$ indicate word-level affinities of original sentences and is used as representation for $\mathbf{H}^a$. For the inter-alignment after self-attention, the sum of each representation and its output are taken as input. Each inter-alignment representation contain the information of both sentences. 
% It first lets the mode attend to each sentence to extract the salient features and global semantics, and then conduct cross-attention to get the aligned representations. 
The model first computes self-alignment attention on each sequence and updates the original representations to make them self-aware. 
Concretely, assume the inputs for an interaction block are
$\mathbf{H}_a=(\mathbf{h}_{a_1}, ..., \mathbf{h}_{a_i}, ..., \mathbf{h}_{a_m})$ 
and 
$\mathbf{H}_b=(\mathbf{h}_{b_1}, ..., \mathbf{h}_{b_j}, ..., \mathbf{h}_{b_n})$, 
where $m$ and $n$ are the corresponding sequence lengths. 
% First, for sentence $a$, we compute the self-attention matrix $E^k_a \in \mathbb{R}^{m \times m}$. Each element $e^k_{ij}$ is the similarity score between $i$-th and $j$-th token:
For sequence $a$, we first compute a self-attention matrix 
$\mathbf A \in \mathbb{R}^{m \times m}$, where each element $\mathbf{a}_{ij}$ measures the semantic similarity between i-th and j-th tokens. Then we update $\mathbf{H}_a$ by adding the attention-weighted sum $\overline{\mathbf{H}}_{a}$ to get self-aware representations:

\vspace{-4mm}
{\fontsize{10}{11}\selectfont
\begin{align}
&\mathbf a_{ij} = F_{1}(\mathbf{h}_{a_i})^\mathrm{T} F_{1}(\mathbf{h}_{a_j}) \\
&\overline{\mathbf{h}}_{a_i} = {\sum_{j=1}^{m}}
{
\frac{exp(\mathbf a_{ij})}{\sum_{k=1}^{m}{exp(\mathbf a_{ik})}}
}
\mathbf{h}_{a_j} \\
&\mathbf{h}^{\prime}_{a_i} = \mathbf{h}_{a_i} + \overline{\mathbf{h}}_{a_i}
\end{align}
\vspace{-5mm}
}

where $F_{1}$ is a feed-forward neural network with ReLU activation. We utilize the same operation for sentence \textit{b} to calculate the self-aware representation ${\mathbf{H}}^{\prime}_b$. After this, a cross-attention layer is applied on ${\mathbf{H}}^{\prime}_a$ and ${\mathbf{H}}^{\prime}_b$ to compute cross-attention matrix $\mathbf E \in \mathbb{R}^{m \times n}$, and then produce the aligned representation $\mathbf{H}^{\prime\prime}_{a}$ and $\mathbf{H}^{\prime\prime}_{b}$:

\vspace{-4mm}
{\fontsize{10}{11}\selectfont
% \setlength{\abovedisplayskip}{2pt}
% \setlength{\belowdisplayskip}{2pt}
\begin{align}
&\mathbf e_{ij} = F_{2}(\mathbf{h}^{\prime}_{a_i})^\mathrm{T} F_{2}(\mathbf{h}^{\prime}_{b_j}) \\
&\mathbf{h}^{\prime\prime}_{a_i} = {\sum_{j=1}^{n}}
{
\frac{exp(\mathbf e_{ij})}{\sum_{k=1}^{n}{exp(\mathbf e_{ik})}}
}
{\mathbf{h}^{\prime}_{b_j}} \\
& \mathbf{h}^{\prime\prime}_{b_j} = {\sum_{i=1}^{m}}
{
\frac{exp(\mathbf e_{ij})}{\sum_{k=1}^{m}{exp(\mathbf e_{kj})}}
}
{\mathbf{h}^{\prime}_{a_i}}
\end{align}
\vspace{-4mm}
}

where $F_{2}$ is another feed-forward neural network with ReLU activation. Intuitively,
self-attention enables model to identify salient contextual features and incorporate these features when computing the cross-attention matrix $\mathbf E$. By doing this the model can properly align the semantic components from two sequences, and thus conduct a better reasoning process for learning their relationship. This is also in line with human behaviors in which people first read each sentence and extract the important content features, and then compare between the two sentences for their relationship.

\smallskip
\noindent \textbf{Gate Fusion Layer.} 
% \yucomment{I think it would be great if we could have a figure showing the work flow of the gate fusion.}
% In order for better information conduction through multiple interaction blocks, we utilize gated fusion mechanism to selectively feed inter-alignment information to next self-aware block.  Suppose the output of block $m$ for $\mathbf{H}^0_a$ is $\mathbf{H}^0{_a_m}$, one of the inputs $input_m$ for the gate fusion module of block $m$ is the concatenation of $\mathbf{H}^0_{a_{m-1}}$ and its encoding(???). Note that $[\mathbf{H}^0_{a_{m-1}}; Encoding(\mathbf{H}^0_{a_{m-1}})]$ is also the input for self-aware alignment module, as described in last paragraph. Another input to gate fusion is the alignment vector $alignment vector_a$ of $\mathbf{H}^0_a$. The gate fusion operations can be described as below.
% % 插入式子
% \begin{align}
% &X = x; x - align; x \circ align \\
% &g_1 = Relu(W^T_1 \cdot X + b_1) \\ 
% &g_2 = Relu(W^T_2 \cdot X + b_2) \\ 
% &g_3 = Relu(W^T_3 \cdot X + b_3) \\ 
% &g_4 = Relu(W^T_4 \cdot X + b_4) \\ 
% &f_1 = Sigmoid(g_1 + g_2) \\ 
% &f_2 = Sigmoid(g_3 + g_4) \\ 
% &\mathbf{H}^0_{a_{m}} = f_1 \cdot x + f_2 \cdot X \\
% \end{align}
% % 解释式子
% $f_1$ controls how much of outputs of last block can be retained. $f_2$ decides how much of the alignment produced by current block $X$ can be retained.
% We design a gate fusion layer to compare and enrich the aligned representations to the original sequences. 
We design a gate fusion layer to compare the original sequences against the aligned representations and blend them together as new sequence representations. 
Specifically, we first conduct a Full Fusion as \newcite{yang-etal-2019-simple} that compares the original representation ($\mathbf{H}_{a}$) with the aligned one ($\mathbf{H}^{\prime\prime}_{a}$) in three perspectives:

\vspace{-4mm}
{\fontsize{10}{11}\selectfont
% \setlength{\abovedisplayskip}{2pt}
% \setlength{\belowdisplayskip}{2pt}
\begin{align}
&{\mathbf{\widetilde{h}}}^{1}_{a_i} = G_1([\mathbf{h}_{a_i}; \mathbf{h}^{\prime\prime}_{a_i}]) \\
&{\mathbf{\widetilde{h}}}^{2}_{a_i} = G_2([\mathbf{h}_{a_i}; \mathbf{h}_{a_i} - \mathbf{h}^{\prime\prime}_{a_i}]) \\
&{\mathbf{\widetilde{h}}}^{3}_{a_i} = G_3([\mathbf{h}_{a_i}; \mathbf{h}_{a_i} \odot \mathbf{h}^{\prime\prime}_{a_i}]) 
% &{\mathbf{\widetilde{h}}}_{a_i} = G([{\mathbf{\widetilde{h}}}^{1}_{a_i};{\mathbf{\widetilde{h}}}^{2}_{a_i};{\mathbf{\widetilde{h}}}^{3}_{a_i}]) \label{eq:full_att}
\end{align}
\vspace{-5mm}
}

where $\odot$ donates element-wise multiplication, $G_1$, $G_2$ and $G_3$ are single layer feed-forward networks with different parameters, and $[;]$ donates concatenation. By this operation both similarity (by multiplication) and difference (by subtraction) of two representations are measured. Then the three perspectives are combined with a non-linear transformation:

\vspace{-4mm}
{\fontsize{10}{11}\selectfont
\begin{align}
&{\mathbf{\widetilde{h}}}_{a_i} = ReLU(\mathbf{W_f}[{\mathbf{\widetilde{h}}}^{1}_{a_i};{\mathbf{\widetilde{h}}}^{2}_{a_i};{\mathbf{\widetilde{h}}}^{3}_{a_i}] + \mathbf{b_f}) \label{eq:full_att}
\end{align}
\vspace{-5mm}
}

where $\mathbf{W_f}$ and $\mathbf{b_f}$ are trainable parameters. Also, different from the popular LSTM-based fusion layers~\cite{wang-jiang-2016-learning,rocktaschel2015reasoning}, this operation helps to reduce the computational complexity.

% where $\odot$ donates element-wise multiplication, $G_1$, $G_2$, $G_3$ and $G$ are single layer feed-forward networks with different parameters, and $[;]$ donates concatenation. By this operation both similarity (by multiplication) and difference (by subtraction) of two representations are measured. Also, different from the popular LSTM-based fusion layers~\cite{wang-jiang-2016-learning,rocktaschel2015reasoning}, this operation helps to reduce the computational complexity.


Since the original sequence representations contain more global semantic information, we further apply a gated connection to enable model selectively integrate the aligned features, which is implemented as:

\vspace{-5mm}
{\fontsize{10}{11}\selectfont
% \setlength{\abovedisplayskip}{2pt}
% \setlength{\belowdisplayskip}{2pt}
\begin{align}
& f_i = \sigma(
\mathbf{W}_{1}\mathbf{h}_{a_i} +
\mathbf{W}_{2}{\mathbf{\widetilde{h}}}_{a_i} +
\mathbf{b_g}
) \\
&\widehat{\mathbf{h}}_{a_{i}} = f_i \cdot \mathbf{h}_{a_i} +
(1 - f_i) \cdot {\mathbf{\widetilde{h}}}_{a_i}
\end{align}
}
\vspace{-6mm}

where $\mathbf{W}_{*}$ and $\mathbf{b_g}$ are trainable parameters, and $\sigma$ is a sigmoid nonlinear transformation. The same operation is conducted on sentence b, thus having the outputs $\widehat{\mathbf{H}}_{a}$ and $\widehat{\mathbf{H}}_{b}$. By doing this, model can flexibly interpolate the aligned information to the original representations through setting the gate, especially when multiple interaction blocks are applied.
% Especially when multiple interaction blocks are applied, model can decide how much aligned information in different levels to be propagated to the following layers.
Also, this is similar as a skip connection which can prevent the additional model complexity coming from stacked interactions and reduce the training difficulty. We discuss how gate operation enables deeper structures with stacked interaction blocks in Section \ref{ablation}.
% Also, in the case of multiple interaction blocks are stacked, the model will learn how much new information from different levels of interactions to integrate to the original representations by setting the gates.


\subsection{Aggregation Layer}\label{Aggregation Layer}
% We apply an aggregation layer to produce the final representations for each sentence on the top of interaction blocks. A convolutional neural network (with padding) is used to obtain high-level semantic representations. 
We apply a convolutional neural network (with padding) to obtain high-level semantic representations for each sentence on the top of interaction blocks. 
% Formally, given the outputs of the last interaction blocks: $\mathbf{H}^k_a=[\mathbf{h}^k_{a_1}, ..., \mathbf{h}^k_{a_i}, ..., \mathbf{h}^k_{a_m}]$ and $\mathbf{H}^k_b=[\mathbf{h}^k_{b_1}, ..., \mathbf{h}^k_{b_i}, ..., \mathbf{h}^k_{b_m}]$, we get the aggregated representations:
Formally, given the outputs of the interaction blocks, we get the aggregated representations:

\vspace{-5mm}
{\fontsize{10}{11}\selectfont
% \setlength{\abovedisplayskip}{2pt}
% \setlength{\belowdisplayskip}{2pt}
\begin{align}
&\mathbf{V}_a = CNN(\mathbf{U}_a) \\
&\mathbf{V}_b = CNN(\mathbf{U}_b)
\end{align}
\vspace{-6mm}
}

where $\mathbf{U}_a$, $\mathbf{U}_b$ are the outputs of the last interaction block, and $\mathbf{V}_a$, $\mathbf{V}_b$ are the aggregated sentence representations and will be used as the inputs for the prediction layer.


\subsection{Prediction Layer}\label{Prediction Layer}
To get the vector representations of each sequence, we apply mean and max pooling on $\mathbf{V}_a$ and $\mathbf{V}_b$~\cite{liang-etal-2019-asynchronous} to produce both global and salient semantic features:
% The final combined feature vector is obtained by the concatenation of different operations as~\cite{liang-etal-2019-asynchronous}:

\vspace{-5mm}
{\fontsize{10}{11}\selectfont
% \setlength{\abovedisplayskip}{2pt}
% \setlength{\belowdisplayskip}{2pt}
\begin{align}
&\mathbf{V}^{mean}_{a} = \frac{1}{m}{\sum_{i=1}^{m}{\mathbf{v}_{a_i}}}, \mathbf{V}^{max}_{a} = \max_{i=1}^{m}{\mathbf{v}_{a_i}} \\
&\mathbf{V}^{mean}_{b} = \frac{1}{n}{\sum_{j=1}^{n}{\mathbf{v}_{b_j}}}, \mathbf{V}^{max}_{b} = \max_{j=1}^{n}{\mathbf{v}_{b_j}} \\
& \mathbf{V}^{\prime}_{a}=[\mathbf{V}^{mean}_{a};\mathbf{V}^{max}_{a}], \mathbf{V}^{\prime}_{b}=[\mathbf{V}^{mean}_{b};\mathbf{V}^{max}_{b}] 
\end{align}
\vspace{-5mm}
}

\noindent Then we combined $\mathbf{V}^{\prime}_{a}$ and $\mathbf{V}^{\prime}_{b}$ to produce the final feature vector by concatenating the different operations:

\vspace{-5mm}
{\fontsize{10}{11}\selectfont
% \setlength{\abovedisplayskip}{2pt}
% \setlength{\belowdisplayskip}{2pt}
\begin{align}
&\mathbf{V}=[\mathbf{V}^{\prime}_{a};\mathbf{V}^{\prime}_{b};
\mathbf{V}^{\prime}_{a} - \mathbf{V}^{\prime}_{b}; \mathbf{V}^{\prime}_{a} \odot \mathbf{V}^{\prime}_{b}]
\end{align}
\vspace{-6mm}
}

\noindent Finally the prediction layer takes as input the feature vector  $\mathbf{V}$, and passes it to a multi-layer feed-forward neural network (MLP) to calcuate the final target. Softmax is applied onto the final layer to get the probability distributions for each class. 


==> EMNLP 2021 COIN-camera-ready/intro.tex <==
Semantic text matching is among the most fundamental tasks in natural language processing. Given two sentences, the goal is to predict their semantic relationship. In this work, we focus in particular on question matching (QM) benchmarks.

Recently, the availability of large-scale annotated datasets has led to a proliferation of deep neural architectures for text matching~\cite{williams-etal-2018-broad,chen-etal-2017-enhanced,wang2017bilateral}. Most existing neural models fall into two categories, namely the sentence encoding and the sentence interaction approaches~\cite{lan-xu-2018-neural}. The former encodes sentences as fixed-length vector representations, which are then consulted to make the final prediction. The latter considers interactions between two sequences to identify their semantic connections, which tends to yield better results.



\begin{figure}[t]
    \centering
    \includegraphics[scale=0.38]{fig/attention_description.pdf}
    \vspace{-2mm}
    \captionof{figure}{ 
    The original attention mechanism (left) and the proposed context-aware attention (right). 
    $w_{*}$ represents the two sequences (more generally, they can be regarded as query and key). $C_{*}$ denotes the contextual features.
    }
    \label{fig:att_descript}
    \vspace{-4mm}
\end{figure}

Attention mechanisms are widely adopted for the sentence-interaction approaches, relying on a word-by-word attention matrix to obtain alignment information between two sequences. This has proven fruitful in modeling sentence pair relationships~\cite{parikh-etal-2016-decomposable,rocktaschel2015reasoning,wang-jiang-2016-learning}.
Nonetheless, when computing the cross-sentence attention, existing models mostly focus on word-level local matching and fail to fully account for 
the overall semantics: \textit{each value of the attention matrix is based on just two individual tokens from the sequences without full consideration of the context}. 
As shown in Figure~\ref{fig:att_descript}, in the original attention mechanism, each token individually attends to the other tokens without accounting for important contextual information. 
However, accurate matching may require a deeper understanding of the two sentences along with pertinent linguistic patterns and constructions~\cite{storks2019recent}.
\newcite{yang2019context} show that 
contextualizing the self-attention network may improve the original representations, but they do not consider the scenario of 
sentence pairs with cross-attention.


In this work, we aim to generalize the notion of cross-sentence attention by enabling it to incorporate rich contextual signals. We propose a 
\underline{CO}ntext-aware \underline{I}nteraction \underline{N}etwork
(\textbf{COIN}) with a novel \textit{context-aware attention layer}. 
This layer enables the model to consult contextual information while computing the cross-attention matrix to measure the word relevance, yielding
better contextualized alignments for semantic reasoning.
We leverage the self-alignment on each sequence to produce contexts that represent salient features for each token. The subsequent gate fusion layer is designed to enable the model to selectively integrate the aligned representations and control to what extent the new information is to be passed to the following layers, which is similar to a skip connection in mitigating the additional model complexity coming from the deeper structure. Finally, an aggregation layer and a multi-head pooling layer are adopted to infer high-level semantic representations for the sequences and predict the result based on the refined representations.

To validate the effectiveness of our method, we conduct extensive experiments on the Quora and LCQMC datasets, along with further analyses of model components and a case study visualizing the alignment. The results show that by incorporating rich context into cross-attention, our model outperforms state-of-the-art methods without the huge number of model parameters and pre-training on extrinsic data of BERT models.

==> EMNLP 2021 COIN-camera-ready/model.tex <==

Question matching can be viewed as a classification task that seeks a label $y \in \mathcal{Y}= \{\textsc{Duplicate}, \textsc{Non-Duplicate}\}$ for a given sentence pair $(S_a, S_b)$. Figure~\ref{fig:model_structure} illustrates our novel sentence interaction approach for this task. In the following, we describe the individual ingredients of this approach.

\subsection{Input Representation Layer}
The input representation layer converts each sentence into matrix representations with an embedding and encoding layer. We invoke word embeddings without additional lexical features and adopt a multi-layer convolutional encoder on top of the embedding layer. In addition, we concatenate the contextual representations with the original embeddings to produce better alignments in the following interaction blocks. This serves a similar purpose as skip connections to represent words at different levels~\cite{wang-etal-2018-multi}.

\subsection{Context-aware Interaction Block}\label{Self-aware Interaction Block}
Our proposed interaction block consists of a context-aware cross-attention and a gate fusion layer. Several such interaction blocks are stacked to obtain refined alignments.
\subsubsection{Cross-Attention Layer} 
We first review the original cross-sentence attention before introducing our context-aware form of attention. Assume the two inputs of the current layer are
$\mathbf{H}_a=(\mathbf{h}_{a_1}, ..., \mathbf{h}_{a_m})$ 
and 
$\mathbf{H}_b=(\mathbf{h}_{b_1}, ..., \mathbf{h}_{b_n})$, 
where $m$ and $n$ are the corresponding sequence lengths. The word-by-word attention matrix is first calculated as follows: 

\vspace{-4mm}
{\fontsize{10}{11}\selectfont

\begin{align}
&\mathbf E_{ij} = {\rm Att}(\mathbf{h}_{a_i}, \mathbf{h}_{b_j}) = F_{1}(\mathbf{h}_{a_i})^\mathrm{T} F_{1}(\mathbf{h}_{b_j}), \label{eq:attention}\vspace{-5mm}
\end{align}%
}%
\noindent where $F_1$ is a feed-forward neural network. Then the similarity matrix $\mathbf E$ is used to compute aligned representations of each sequence as a weighted summation with regard to the other sentence:

\vspace{-4mm}
{\fontsize{10}{11}\selectfont
\begin{align}
&\mathbf a_{i} = \rm softmax(\mathbf E_{i:}),\quad \mathbf b_{j} = \rm softmax(\mathbf E_{:j}) \\
& \mathbf{h}^{\prime}_{b_j} = {\sum_{k=1}^{m}}{\mathbf b_{kj} \mathbf h_{a_k}},\quad \mathbf{h}^{\prime}_{a_i} = {\sum_{k=1}^{n}}{\mathbf a_{ik} \mathbf h_{b_k}}\vspace{-5mm}
\end{align}%
}\vspace{-4mm}

\noindent \textbf{Limitation.} It is evident in Eq.~\ref{eq:attention} that each value of the attention matrix is governed by the parameters of the feed-forward layer with respect to only the individual token pairs, 
so the layer does not take advantage of valuable contextual signals.

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.58]{fig/model-coin-large-2.pdf}
    \captionof{figure}{ 
    Overview of our model structure.
    }
    \label{fig:model_structure}
\end{figure}

\subsubsection{Context-Aware Cross-Attention Layer} 
We propose a novel context-aware cross-attention layer by incorporating  contextual representations into the cross-attention. The goal is to enable the model to identify salient contextual features for each token, and consider these features when computing the cross-attention matrix $\mathbf E$. 

Given $\mathbf C_{a}= (\mathbf c_{a_1}, ..., \mathbf c_{a_m})$, $\mathbf C_{b}=(\mathbf c_{b_1}, ..., \mathbf c_{b_n})$ as contextual representations for the two sentences, we modify the attention mechanism from Eq.~\ref{eq:attention} to be able to draw on these as additional inputs when computing the word-by-word attention matrix:

\vspace{-2mm}
{\fontsize{10}{11}\selectfont
\begin{align}
\begin{split}
\mathbf E^\mathrm{c}_{ij} &= {\rm Att_{context}}(\mathbf{h}_{a_i}, \mathbf{h}_{b_j}, \mathbf{c}_{a_i}, \mathbf{c}_{b_j}) \\
&= F_{1}(\mathbf{h}_{a_i} + \mathbf{c}_{a_i} )^\mathrm{T} F_{1}(\mathbf{h}_{b_j} + \mathbf{c}_{b_j})
\end{split}\vspace{-1mm}
\end{align}%
%
}%

\noindent By incorporating the contextual vectors, the model is able to take advantage of the full context and enable better alignments. 

\smallskip
\noindent \textbf{Contextual Representations.} In order to compute such representations of the contexts, given each sequence, we adopt a self-alignment layer to aggregate pertinent contextual information. Each contextual vector is computed by attending to the input hidden states and conducting a weighted summation. Formally, for the input $\mathbf H = (\mathbf{h}_1, ..., \mathbf{h}_n)$:

\vspace{-2mm}
{\fontsize{10}{11}\selectfont
\begin{align}
&\mathbf A = {\rm ReLU}(\mathbf W_c\mathbf H)^\mathrm{T}\, {\rm ReLU}(\mathbf W_c\mathbf H) \\
&\mathbf C = \rm softmax(\mathbf A) \mathbf H
\end{align}
\vspace{-4mm}
}

\noindent Here, $\mathbf{W}_c$ is a trainable parameter. 


Leveraging the self-alignment to produce contextual signals also mirrors human behavior in the sense that when matching two sentences, people tend to first process each sentence paying attention to the important contents, and then compare the two sentences and connect relevant elements (words or phrases) with contextual features to identify their relationship, rather than just comparing individual words.


\subsubsection{Gate Fusion Layer} 
Subsequently, a gate fusion layer compares the original sequences against the aligned representations and blends them together as new sequence representations. 
Specifically, we first compare the original representation ($\mathbf{H}_{a}$) with the aligned one ($\mathbf{H}^{\prime}_{a}$) from three perspectives, and then combine them with a non-linear transformation:

\vspace{-5mm}
{\fontsize{10}{11}\selectfont

\begin{align}
&{\mathbf{\widetilde{h}}}^{1}_{a_i} = G_1([\mathbf{h}_{a_i}; \mathbf{h}^{\prime}_{a_i}]) \label{eq:ori}\\
&{\mathbf{\widetilde{h}}}^{2}_{a_i} = G_2([\mathbf{h}_{a_i}; \mathbf{h}_{a_i} - \mathbf{h}^{\prime}_{a_i}]) \\
&{\mathbf{\widetilde{h}}}^{3}_{a_i} = G_3([\mathbf{h}_{a_i}; \mathbf{h}_{a_i} \odot \mathbf{h}^{\prime}_{a_i}]) \\
&{\mathbf{\widetilde{h}}}_{a_i} = \mathrm{ReLU}(\mathbf{W}_f[{\mathbf{\widetilde{h}}}^{1}_{a_i};{\mathbf{\widetilde{h}}}^{2}_{a_i};{\mathbf{\widetilde{h}}}^{3}_{a_i}] + \mathbf{b}_f)
\label{eq:sim}
\end{align}
\vspace{-6mm}
}

\noindent 
Then a gated connection is applied to enable the model to selectively integrate the aligned features:
\newcommand{\vect}[1]{\boldsymbol{#1}}
\vspace{-6mm}
{\fontsize{10}{11}\selectfont

\begin{align}
& \vect{f}_i = \sigma(
\mathbf{W}_{1}\mathbf{h}_{a_i} +
\mathbf{W}_{2}{\mathbf{\widetilde{h}}}_{a_i} +
\mathbf{b}_g
) \\
&\widehat{\mathbf{h}}_{a_{i}} = \vect{f}_i \odot \mathbf{h}_{a_i} +
(\mathbf1 - \vect{f}_i) \odot {\mathbf{\widetilde{h}}}_{a_i}
\end{align}
}
\vspace{-6mm}

\noindent Here $\sigma$ is a Sigmoid nonlinear transformation, while $\mathbf{W}_{\ast}$ and $\mathbf{b}_g$ are trainable parameters. The same operation is conducted on sentence $S_b$, thereby yielding the outputs $\widehat{\mathbf{H}}_{a}$ and $\widehat{\mathbf{H}}_{b}$. With these operations, the model can flexibly interpolate the aligned information by controlling the gate, especially when multiple interactions are applied.



\subsection{Aggregation Layer}\label{Aggregation Layer}
To obtain high-level semantic representations for each sentence, we apply another convolutional neural network on top of the interaction blocks to obtain the aggregated sentence representations $\mathbf{V}_a$, $\mathbf{V}_b$, serving as the inputs for the prediction layer.


\subsection{Pooling and Prediction Layer}\label{Prediction Layer}
We compute a weighted summation of the hidden states to get sentence vectors.
To allow the model to represent each sequence in different representation subspaces, we adopt multi-head pooling following \newcite{liu-lapata-2019-hierarchical}. For each head $z$, we first transform the sequence into attention scores $\mathbf S^z$ and values $\mathbf{\widetilde V}^z$:

\vspace{-6mm}
{\fontsize{10}{11}\selectfont

\begin{align}
& \mathbf S^z = {\rm softmax}(\mathbf W^z_a\mathbf V_a) \\
& \mathbf{\widetilde V}^z = \mathbf{W}^z_v\mathbf{V}_{a}
\end{align}
\vspace{-6mm}
}

\noindent where $\mathbf W^z_a \in \mathbb{R}^{1 \times d}$ and $\mathbf W^z_u \in \mathbb{R}^{d_\mathrm{h} \times d}$ are trainable parameters,  with $d_\mathrm{h} = d / n_\mathrm{h}$ as the dimensionality of each head and $n_\mathrm{h}$ as the number of heads. The pooling vector of head $z$ is
computed as

\vspace{-4mm}
{\fontsize{10}{11}\selectfont
\begin{align}
& {\mathbf{\widehat V}^z} = {\sum_{i=1}^{n}}{{\mathbf s^z_i}{\mathbf {\widetilde v}^z_i}},
\end{align}
\vspace{-4mm}
}

\noindent where $\mathbf s^z_i$ and $\mathbf {\widetilde v}^z_i$ denote the calculated attention scores and values. 
The pooling vectors of all heads are  concatenated to form the final vector representations of each sequence $\mathbf{V}^{\prime}_{a}$ and $\mathbf{V}^{\prime}_{b}$. We combine $\mathbf{V}^{\prime}_{a}$ and $\mathbf{V}^{\prime}_{b}$ to produce the overall representation by concatenating the different operations:

\vspace{-4mm}
{\fontsize{10}{11}\selectfont

\begin{align}
&\mathbf{V}=[\mathbf{V}^{\prime}_{a};\mathbf{V}^{\prime}_{b};
\mathbf{V}^{\prime}_{a} - \mathbf{V}^{\prime}_{b}; \mathbf{V}^{\prime}_{a} \odot \mathbf{V}^{\prime}_{b}]
\end{align}
\vspace{-4mm}
}

\noindent Finally, the prediction layer takes the representation $\mathbf{V}$ and passes it to a fully-connected network component to predict the ultimate target scores. 


==> EMNLP 2021 COIN-camera-ready/related.tex <==



The task of natural language inference or textual entailment recognition has a long history in natural language processing. 
Early explorations relied on hand-crafted features and traditional NLP pipeline approaches \cite{maccartney-manning-2008-modeling,heilman2010tree}. 

Recent deep neural network models have shown promising results in this area with the availability of large-scale datasets~\cite{bowman-etal-2015-large,williams-etal-2018-broad,khot2018scitail,wang2020multi,peng2020enhanced}. 
In this regard, the conceptually simpler sentence encoding approach aims to first learn good sentence representations and then makes a prediction based on the combination of sentence representations~\cite{mou-etal-2016-natural,conneau-etal-2017-supervised,yin-schutze-2015-convolutional}. However, such models neglect fine-granular sentence interaction information. The sentence interaction approach instead adopts an attention mechanism to match the two sequences and subsequently aggregates the aligned features to obtain high-level representations and predictions. \newcite{wang-jiang-2016-learning} use a match-LSTM to perform word-by-word matching of the hypothesis with the premise. \newcite{parikh-etal-2016-decomposable} employ a decomposable attention method that computes word pair interactions and soft alignments. BiMPM~\cite{wang2017bilateral} matches the two encoded sentences in two directions with a multi-perspective matching operation, and aggregates the matching results with another Bi-LSTM. Nonetheless, these architectures remain relatively shallow and have trouble capturing more complex semantic relations.

The DIIN  model~\cite{gong2017natural} solves text matching tasks by extracting semantic features from an interaction space, and adopts a DenseNet as a convolutional feature extractor. \newcite{chen-etal-2018-neural-natural} propose a knowledge-based inference model with enrichment of external knowledge in calculating coattention, collecting local inferences, and composing the inference. RE2~\cite{yang-etal-2019-simple} has shown strong performance and fast inference speed by focusing on three forms of interaction features.
\newcite{duan2018attention} leverages a deep structure with joint cross-attention and self-attention. However, context features are not well considered when computing cross-sentence attention in the aforementioned systems.

Recently pre-trained language models have been in the center of attention, trained on large-scale corpora and subsequently fine-tuned for various downstream tasks~\cite{devlin-etal-2019-bert,liu2019roberta,sun2019ernie}. Despite achieving promising performance on many natural language understanding problems, these architectures usually have a large parameter size and are hard to be deployed in many applications with the requirement of inference speed. 
Also, they only adopt self-attention over the concatenation of two sequences, and it is unclear whether inter-alignment can be effectively learned.
Our work adopts an interaction-based structure to model sentence relationships and achieves comparative results while maintaining less computational complexity.

Multi-hop attention mechanisms have yielded improvements on machine comprehension~\cite{gong-bowman-2018-ruminating,wang-etal-2018-multi} and implicit argument prediction~\cite{cheng2019implicit}. Different from the above methods, our two-hop attention mechanism consists of self-attention and cross-attention, which strengthens the model's capacity to capture salient contextual information for a proper alignment. A gate fusion layer is adopted to flexibly integrate the aligned representations, and multiple interaction blocks are stacked to conduct alignments at multiple scales.


==> fig/intro.tex <==
Natural language inference, which is also known as recognizing textual entailment (RTE), is a fundamental task in natural language processing. Given a premise sentence and a hypothesis sentence, the model needs to predict whether the premise can infer the hypothesis~\cite{bowman-etal-2015-large}. 
This is a challenging task because it requires model to deeply understand the texts, capture proper language patterns, and conduct correct logical reasoning in different levels which also relies on commonsense knowledge~\cite{storks2019recent}. 
% \yucomment{change to: it requires model to capture language patterns and text relatedness in different levels (\ie word-, and sentence- level)?}

% \begin{figure}[t]
%     \def\arraystretch{1.1}
%     \bgroup
%     % \def\arraystretch{1.1}
% 	\fontsize{9}{10}\selectfont
%      \hspace{-1mm}
% 	\setlength{\tabcolsep}{0.8mm}
% 	\begin{tabular}{|p{75mm}|}
% 	\hline
% % 	\vspace{0.03mm}
% 	\textbf{Premise}: A group of kids is splashing in deep water nearby a rock formation. \\
% 	\textbf{Hypothesis}: The kids are in deep water. \\
% 	\textbf{Label}: \textit{Entailment} \\
% 	\\
% 	\textbf{Premise}: A busy street with numerous people interacting and going about their lives. \\
% 	\textbf{Hypothesis}: The morning rush hour fills the streets with busy people. \\
% 	\textbf{Label}: \textit{Neutral} \\ 
% 	\vspace{0.3mm}
% 	\textbf{Premise}: The little boy gets ready to kick the soccer ball. \\
% 	\textbf{Hypothesis}: The boy is sleeping at home. \\
% 	\textbf{Label}: \textit{Contradiction} \\
	
% 	\hline
% % 	\vspace{0.03mm}
% 	\textbf{Text1}: What should I do to avoid sleeping in class? \\
% 	\textbf{Text2}: How do I not sleep in a boring class? \\
% 	\textbf{Label}: \textit{Paraphrase} \\
% 	\\
% 	\textbf{Text1}: What is the best time to read MBA? \\
% 	\textbf{Text2}: What 's the best time for reading? \\
% 	\textbf{Label}: \textit{Non-paraphrase} \\
%     \hline
	
% 	\end{tabular}
%     \vspace{-3mm}
% \caption{Examples for natural language inference and paraphrase identification. The samples in the upper box are taken from SNLI dataset, and in the bottom box are from Quora dataset.} 
% \label{fig:sample-keyphrase}
% \egroup
% \vspace{-5mm}
% \end{figure}


% \begin{figure*}[t]
%     \centering
%     \includegraphics[scale=0.6]{fig/model_figure2.pdf}
%     \captionof{figure}{ 
%     Our proposed model structure. On the left is the main framework of SENAN, which has 4 parts: a representation layer, multiple stacked interactions blocks, a aggregation layer and a final prediction layer. On the right is detailed structure of the self-aware interaction block consisting of a two-hop attention and a gate fusion operation.
%     \todo{modify the figure color}
%     }
%     \label{fig:model_structure}
%     % \vspace{-4mm}
% \end{figure*}

Recently neural network approaches have been successfully applied to NLI with the availability of large-scale annotated datasets and the development of deep learning techniques~\cite{bowman-etal-2015-large,williams-etal-2018-broad,chen-etal-2017-enhanced,wang2017bilateral,wang-jiang-2016-learning}. Most existing neural models fall into two types, namely sentence encoding approach and sentence interaction approach. The former encodes sentences into vector representations and makes the prediction based on them, while the latter considers interactions between two sequences to capture their semantic relations and usually achieves better results.


Attention mechanism has been widely adopted in sentence interaction approach where a word-by-word attention matrix is computed to get aligned information between two sequences. This method has been proved to be useful to address NLI task~\cite{gong2017natural,parikh-etal-2016-decomposable,rocktaschel2015reasoning,wang-jiang-2016-learning}.
% \yucomment{change to: This method has proved useful to address the text matching task.}
Nevertheless, when computing the word-level cross sentence attention, existing models only focus on local matching and insufficiently consider global semantics: each element of the attention matrix is calculated by two individual tokens from the sequences without direct consideration of the global contexts. 
% \yucomment{It's not clear what are you trying to say in the rest of this paragraph. Is this a second motivation? Or is it the solution you proposed?} 

When human conduct this task, they tend to first go through each sentence and pay attention to the salient contents (similar as conducting self-attention on each sequence), and then compare against the other sentence and connect the relevant elements such as words or phrases to learn their relations (can be viewed as cross-attention between two sequences). Usually this procedure is conducted for multiple times to get a better understanding of the sentence relationship, and then make the final prediction.

Inspired by this, we propose a 
\underline{SE}lf-aware I\underline{N}ter\underline{A}ction \underline{N}etwork
(SENAN) with a novel self-aware interaction block to capture sequence relations and update the sentence representations, as shown in Figure~\ref{fig:model_structure}. Concretely, the self-aware interaction block consists of a two-hop attention and a gate fusion layer. 
In two-hop attention, the model first computes self-alignment attention for each sequence to enrich the original representations with salient contextual features, and then conducts a cross sentence attention to produce proper alignments for semantic reasoning.
The gate fusion layer is designed to enable model to selectively integrate the aligned representations and control how much the new information to be passed to the following layers. 
In addition, We apply stacked interaction blocks to strength the model ability on refining the attention distributions and updating sentence representations progressively. This forms a 
\textbf{multi-step reasoning process}. We then adopt an aggregation layer to produce high-level semantic representations for the premise and hypothesis, and predict the result based on the refined representations. 

To validate the effectiveness of our proposed method, we conduct extensive experiments on SNLI, MultiNLI, SciTail and Quora Questions Pairs datasets, and provide analysis on model components and a case study through visualization of alignment results\footnote{We will release our code upon publication.}. The overall contributions of our work can be summarized as follows:
\begin{itemize}
% \smallskip
\item We propose a novel self-aware interaction network with a two-hop attention to produce proper alignments between two sequences. The multiple interactions are applied to let model gradually learn semantic relatedness and refine attention results.

\item We design a gate fusion layer to flexibly integrate the aligned features and update sequence representations from different levels. 
% The gate mechanism can be also viewed as a shortcut connection to reduce the training difficulty. 
An aggregation layer is applied to produce high-level semantic representations of each sentences for prediction.

\item We evaluate our model capacity on four benchmark NLI (alike)  datasets with extensive experiments. Our approach outperforms strong comparisons with competitive results, which validates the model effectiveness for solving natural language inference task.

% \item We propose a two-hop attention operation which consists of a self-attention and a cross-attention, to capture proper alignments of two sequences. We apply multiple interactions to learn different levels of relatedness and gradually refine the alignment results.

% \item We design a gate fusion to flexibly integrate aligned features and update sequence representations from different levels. An aggregation layer is applied to produce final sequence representations for the prediction.

% \item We evaluate our model capacity on four benchmark datasets, and the results show our approach outperforms strong comparisons with competitive results.
\end{itemize}


==> fig/model.tex <==
% \section{Our Model}
\begin{figure*}[t]
    \centering
    % \includegraphics[scale=0.63]{fig/model_figure5.pdf}
    \includegraphics[scale=0.63]{fig/model-yy.pdf}
    \captionof{figure}{ 
    Our proposed model structure. On the left is the main framework of SENAN, which has 4 parts: a representation layer, stacked interactions blocks, an aggregation layer and a final prediction layer. On the right is detailed structure of the self-aware interaction block consisting of a two-hop attention and a gate fusion layer.
    }
    \label{fig:model_structure}
    \vspace{-5mm}
\end{figure*}

Natural language inference can be viewed as a classification task that predicts the label $Y$ for a given premise-hypothesis pair $(S_a, S_b)$, where $Y$ = \{\textit{entailment}, \textit{contradiction}, \textit{neutral}\}. We propose an interaction based neural approach to tackle this problem as shown in Figure~\ref{fig:model_structure}. 


% Unlike existing models for this task, our model: (1) Consists of self-aware interactions blocks which combines self-attention and inter-sentences alignment; (2) Fuses sentence information and alignment information by a gated fusion layer to let the model flexibly control the information pass to the next layer' (3) Utilizes an aggregation layer after interaction blocks to get the final representation. 

% In our model, each sentence is embedded on both char-level and word-level. The concatenation of both embeddings is then used as input for the encoder, a simple CNN encoder. In order to keep more information before passing through the encoder, instead of only the encoding, the concatenation of embeddings and encoding is fed to a self-aware attentive alignment module. The module is composed of N blocks with identical structures and independent parameters. Each block: (1) is not only consisted of inter-sentence alignment, but also of self-attention of each sentence; (2) uses gated fusion mechanism to incorporate alignments into sentence representations. Details of the alignment module will be discussed below in section **. After the module, alignment representations for each sentence are then aggregated, pooled and fed to classification layer. Except for the alignment layer, symmetric architectures are used for both input sentences, using shared the parameters.

In our approach, each sentence is first embedded and encoded to get the sentence representations. Then we design a self-aware interaction block to properly align two sequences and capture their semantic relatedness for the logical reasoning.
% which consists of (1) a two-hop attention operation with both self-attention and cross-attention,
% and (2) a gate fusion layer to flexibly integrate aligned information.
% , which lets the model flexibly control how much information to be passed to the next layer. 
In addition, we apply multiple interaction blocks with independent parameters to gradually learn semantic relations and reason between two sequences in different levels. Details of the self-aware interaction block will be discussed below in Section \ref{Self-aware Interaction Block}. Then the representations for each sentence are aggregated, pooled and fed to a classification layer. Symmetric architecture is used for both input sentences with shared parameters.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[scale=0.6]{fig/model_figure2.pdf}
%     \captionof{figure}{ 
%     Our proposed model structure. On the left is the main framework of SENAN, which has 4 parts: a representation layer, multiple stacked interactions blocks, a aggregation layer and a final prediction layer. On the right is detailed structure of the self-aware interaction block consisting of a two-hop attention and a gate fusion operation.
%     \todo{modify the figure color}
%     }
%     \label{fig:model_structure}
%     % \vspace{-4mm}
% \end{figure*}

\subsection{Input Representation Layer}

% The encoding layer first converts sentence pairs into embeddings. In our model, both character embeddings and word embeddings are used. Given a sentence pair $Q=[q_w_1, ..., q_w_i, ..., q_w_m]$, $P=[p_w_1, ..., p_w_j, ..., p_w_n]$, where $q_w_i$ and $p_w_j$ denotes the $i$-th and $j$-th word of $Q$ and $P$ respectively, a pre-trained look-up table $M_w$ is leveraged to convert $Q$ and $P$ into vectors. $Q$ and $P$

The input representation layer converts each sentence into matrix representations with an embedding and encoding layer. 

\smallskip
\noindent \textbf{Embedding.} 
In our model, both word embeddings and character embeddings are used. To get the character-based word representations, we apply a convolutional neural network (CNN) with max pooling over the entire tokens ~\cite{kim2016character}. The character embeddings have been shown to be useful for out-of-vocabulary (OOV) problem. For word embeddings, we adopt the commonly used Glove embeddings~\cite{pennington-etal-2014-glove} to represent each token as a vector. Following \newcite{seo2016bidirectional}, the outputs of word embeddings and character embeddings are concatenated, and then passed through a 2-layer highway network~\cite{srivastava2015highway} to get the final representation of each single word. 

\smallskip
\noindent \textbf{Encoding.} To encode the contextual information into token representations, we use a stacked Bidirectional LSTM (Bi-LSTM)~\cite{hochreiter1997long} encoder on the top of the embedding layer to model temporal interactions between words,
% Following \newcite{tay-etal-2018-co}, we apply a stacked recurrent encoder layer,
% Hence we obtain the contextual representations of two sentences
% % $\mathbf{H}_a=[\mathbf{h}_{a_1}, ..., \mathbf{h}_{a_i}, ..., \mathbf{h}_{a_m}]$ and $\mathbf{H}_b=[\mathbf{h}_{b_1}, ..., \mathbf{h}_{b_j}, ..., \mathbf{h}_{b_n}]$, where $\mathbf{H}_a \in \mathbb{R}^{m \times d}$ and $\mathbf{H}_b \in \mathbb{R}^{n \times d}$.
% $\mathbf{H}^0_a=\{\mathbf{h}^0_{a_i}|\mathbf{h}^0_{a_i} \in \mathbb{R}^{2d}, i=1,2,...,m \}$ and $\mathbf{H}^0_b=\{\mathbf{h}^0_{b_j}|\mathbf{h}^0_{b_j} \in \mathbb{R}^{2d}, i=1,2,...,n \}$, where d is the hidden dimension of the forward and backward LSTMs. 
and hence obtain the contextual representations. 
% Inspired by \newcite{yang-etal-2019-simple}, 
In addition, we concatenate the contextual representations with the original embedding vectors to produce better alignments in the following interaction blocks. This is similar as a skip connection to represent words in different levels~\cite{wang-etal-2018-multi}.



\subsection{Self-aware Interaction Block}\label{Self-aware Interaction Block}
% Recently the attention-based neural models have achieved good performance on text matching~\cite{rocktaschel2015reasoning,chen-etal-2017-enhanced,parikh-etal-2016-decomposable,duan2018attention}. 
Our proposed self-aware interaction block consists of
a two-hop attention and a gate fusion layer. The attention is responsible for aligning two sequences and capturing their semantic relationship. 
% We strength the cross-sentence attention to a two-hop style with a self-attention so that the model can better identify the salient contextual features. 
We strength the model with ability to better identify the salient contextual features and properly capture sequence alignments by extending the normal cross-sentence attention to a two-hop style, with an additional self-alignment attention. 
Then the gate fusion layer is leveraged to flexibility integrate the aligned features and update sequence representations.
% to properly capture the alignments between two sequences and selectively integrate the aligned features and update the sequence representations. 
% For the two-hop attention, the model first computes self-attention for each sequence to identify the salient contextual features, and then conducts cross-sentence attention to get aligned representations. 
% By doing this, the model is strengthened with the capacity to better reason between two sentences by capturing the relevant information with salient semantic features. 
% A gate fusion layer is adopted to flexibility fuse the aligned features and update sequence representations.
% \yucomment{change to: A gate fusion layer is adopted to control the amount of information being propagated to the following layers and hence increase the flexibility of the model.} 
In addition, inspired by the idea of end-to-end memory network~\cite{sukhbaatar2015end}, we apply multiple stacked interaction blocks so that our model can gradually refine the alignment results and integrate the inferential information from different levels.

\smallskip
\noindent \textbf{Two-hop Attention.} 
% We applied self-aware alignment to capture semantic features correlated to the relationship of two sentences. Specifically, self-attentive representation of each sentence and inter-alignment are computed. For simplification, we present below the computations on $\mathbf{H}^0_a$. We first concatenate the encoding $\mathbf{H}^0_a$ with its embedding(**Undefined symbol**). The concatenated vectors are then utilized as input for a self attentive representation $\tilde{H}^0_a \in \mathbb{R}^{2d \times 1}$, where $\tilde{H}^0_a$ indicate word-level affinities of original sentences and is used as representation for $\mathbf{H}^a$. For the inter-alignment after self-attention, the sum of each representation and its output are taken as input. Each inter-alignment representation contain the information of both sentences. 
% It first lets the mode attend to each sentence to extract the salient features and global semantics, and then conduct cross-attention to get the aligned representations. 
The model first computes self-alignment attention on each sequence and updates the original representations to make them self-aware. 
Concretely, assume the inputs for an interaction block are
$\mathbf{H}_a=(\mathbf{h}_{a_1}, ..., \mathbf{h}_{a_i}, ..., \mathbf{h}_{a_m})$ 
and 
$\mathbf{H}_b=(\mathbf{h}_{b_1}, ..., \mathbf{h}_{b_j}, ..., \mathbf{h}_{b_n})$, 
where $m$ and $n$ are the corresponding sequence lengths. 
% First, for sentence $a$, we compute the self-attention matrix $E^k_a \in \mathbb{R}^{m \times m}$. Each element $e^k_{ij}$ is the similarity score between $i$-th and $j$-th token:
For sequence $a$, we first compute a self-attention matrix 
$\mathbf A \in \mathbb{R}^{m \times m}$, where each element $\mathbf{a}_{ij}$ measures the semantic similarity between i-th and j-th tokens. Then we update $\mathbf{H}_a$ by adding the attention-weighted sum $\overline{\mathbf{H}}_{a}$ to get self-aware representations:

\vspace{-4mm}
{\fontsize{10}{11}\selectfont
\begin{align}
&\mathbf a_{ij} = F_{1}(\mathbf{h}_{a_i})^\mathrm{T} F_{1}(\mathbf{h}_{a_j}) \\
&\overline{\mathbf{h}}_{a_i} = {\sum_{j=1}^{m}}
{
\frac{exp(\mathbf a_{ij})}{\sum_{k=1}^{m}{exp(\mathbf a_{ik})}}
}
\mathbf{h}_{a_j} \\
&\mathbf{h}^{\prime}_{a_i} = \mathbf{h}_{a_i} + \overline{\mathbf{h}}_{a_i}
\end{align}
\vspace{-5mm}
}

where $F_{1}$ is a feed-forward neural network with ReLU activation. We utilize the same operation for sentence \textit{b} to calculate the self-aware representation ${\mathbf{H}}^{\prime}_b$. After this, a cross-attention layer is applied on ${\mathbf{H}}^{\prime}_a$ and ${\mathbf{H}}^{\prime}_b$ to compute cross-attention matrix $\mathbf E \in \mathbb{R}^{m \times n}$, and then produce the aligned representation $\mathbf{H}^{\prime\prime}_{a}$ and $\mathbf{H}^{\prime\prime}_{b}$:

\vspace{-4mm}
{\fontsize{10}{11}\selectfont
% \setlength{\abovedisplayskip}{2pt}
% \setlength{\belowdisplayskip}{2pt}
\begin{align}
&\mathbf e_{ij} = F_{2}(\mathbf{h}^{\prime}_{a_i})^\mathrm{T} F_{2}(\mathbf{h}^{\prime}_{b_j}) \\
&\mathbf{h}^{\prime\prime}_{a_i} = {\sum_{j=1}^{n}}
{
\frac{exp(\mathbf e_{ij})}{\sum_{k=1}^{n}{exp(\mathbf e_{ik})}}
}
{\mathbf{h}^{\prime}_{b_j}} \\
& \mathbf{h}^{\prime\prime}_{b_j} = {\sum_{i=1}^{m}}
{
\frac{exp(\mathbf e_{ij})}{\sum_{k=1}^{m}{exp(\mathbf e_{kj})}}
}
{\mathbf{h}^{\prime}_{a_i}}
\end{align}
\vspace{-4mm}
}

where $F_{2}$ is another feed-forward neural network with ReLU activation. Intuitively,
self-attention enables model to identify salient contextual features and incorporate these features when computing the cross-attention matrix $\mathbf E$. By doing this the model can properly align the semantic components from two sequences, and thus conduct a better reasoning process for learning their relationship. This is also in line with human behaviors in which people first read each sentence and extract the important content features, and then compare between the two sentences for their relationship.

\smallskip
\noindent \textbf{Gate Fusion Layer.} 
% \yucomment{I think it would be great if we could have a figure showing the work flow of the gate fusion.}
% In order for better information conduction through multiple interaction blocks, we utilize gated fusion mechanism to selectively feed inter-alignment information to next self-aware block.  Suppose the output of block $m$ for $\mathbf{H}^0_a$ is $\mathbf{H}^0{_a_m}$, one of the inputs $input_m$ for the gate fusion module of block $m$ is the concatenation of $\mathbf{H}^0_{a_{m-1}}$ and its encoding(???). Note that $[\mathbf{H}^0_{a_{m-1}}; Encoding(\mathbf{H}^0_{a_{m-1}})]$ is also the input for self-aware alignment module, as described in last paragraph. Another input to gate fusion is the alignment vector $alignment vector_a$ of $\mathbf{H}^0_a$. The gate fusion operations can be described as below.
% % 插入式子
% \begin{align}
% &X = x; x - align; x \circ align \\
% &g_1 = Relu(W^T_1 \cdot X + b_1) \\ 
% &g_2 = Relu(W^T_2 \cdot X + b_2) \\ 
% &g_3 = Relu(W^T_3 \cdot X + b_3) \\ 
% &g_4 = Relu(W^T_4 \cdot X + b_4) \\ 
% &f_1 = Sigmoid(g_1 + g_2) \\ 
% &f_2 = Sigmoid(g_3 + g_4) \\ 
% &\mathbf{H}^0_{a_{m}} = f_1 \cdot x + f_2 \cdot X \\
% \end{align}
% % 解释式子
% $f_1$ controls how much of outputs of last block can be retained. $f_2$ decides how much of the alignment produced by current block $X$ can be retained.
% We design a gate fusion layer to compare and enrich the aligned representations to the original sequences. 
We design a gate fusion layer to compare the original sequences against the aligned representations and blend them together as new sequence representations. 
Specifically, we first conduct a Full Fusion as \newcite{yang-etal-2019-simple} that compares the original representation ($\mathbf{H}_{a}$) with the aligned one ($\mathbf{H}^{\prime\prime}_{a}$) in three perspectives:

\vspace{-4mm}
{\fontsize{10}{11}\selectfont
% \setlength{\abovedisplayskip}{2pt}
% \setlength{\belowdisplayskip}{2pt}
\begin{align}
&{\mathbf{\widetilde{h}}}^{1}_{a_i} = G_1([\mathbf{h}_{a_i}; \mathbf{h}^{\prime\prime}_{a_i}]) \\
&{\mathbf{\widetilde{h}}}^{2}_{a_i} = G_2([\mathbf{h}_{a_i}; \mathbf{h}_{a_i} - \mathbf{h}^{\prime\prime}_{a_i}]) \\
&{\mathbf{\widetilde{h}}}^{3}_{a_i} = G_3([\mathbf{h}_{a_i}; \mathbf{h}_{a_i} \odot \mathbf{h}^{\prime\prime}_{a_i}]) 
% &{\mathbf{\widetilde{h}}}_{a_i} = G([{\mathbf{\widetilde{h}}}^{1}_{a_i};{\mathbf{\widetilde{h}}}^{2}_{a_i};{\mathbf{\widetilde{h}}}^{3}_{a_i}]) \label{eq:full_att}
\end{align}
\vspace{-5mm}
}

where $\odot$ donates element-wise multiplication, $G_1$, $G_2$ and $G_3$ are single layer feed-forward networks with different parameters, and $[;]$ donates concatenation. By this operation both similarity (by multiplication) and difference (by subtraction) of two representations are measured. Then the three perspectives are combined with a non-linear transformation:

\vspace{-4mm}
{\fontsize{10}{11}\selectfont
\begin{align}
&{\mathbf{\widetilde{h}}}_{a_i} = ReLU(\mathbf{W_f}[{\mathbf{\widetilde{h}}}^{1}_{a_i};{\mathbf{\widetilde{h}}}^{2}_{a_i};{\mathbf{\widetilde{h}}}^{3}_{a_i}] + \mathbf{b_f}) \label{eq:full_att}
\end{align}
\vspace{-5mm}
}

where $\mathbf{W_f}$ and $\mathbf{b_f}$ are trainable parameters. Also, different from the popular LSTM-based fusion layers~\cite{wang-jiang-2016-learning,rocktaschel2015reasoning}, this operation helps to reduce the computational complexity.

% where $\odot$ donates element-wise multiplication, $G_1$, $G_2$, $G_3$ and $G$ are single layer feed-forward networks with different parameters, and $[;]$ donates concatenation. By this operation both similarity (by multiplication) and difference (by subtraction) of two representations are measured. Also, different from the popular LSTM-based fusion layers~\cite{wang-jiang-2016-learning,rocktaschel2015reasoning}, this operation helps to reduce the computational complexity.


Since the original sequence representations contain more global semantic information, we further apply a gated connection to enable model selectively integrate the aligned features, which is implemented as:

\vspace{-5mm}
{\fontsize{10}{11}\selectfont
% \setlength{\abovedisplayskip}{2pt}
% \setlength{\belowdisplayskip}{2pt}
\begin{align}
& f_i = \sigma(
\mathbf{W}_{1}\mathbf{h}_{a_i} +
\mathbf{W}_{2}{\mathbf{\widetilde{h}}}_{a_i} +
\mathbf{b_g}
) \\
&\widehat{\mathbf{h}}_{a_{i}} = f_i \cdot \mathbf{h}_{a_i} +
(1 - f_i) \cdot {\mathbf{\widetilde{h}}}_{a_i}
\end{align}
}
\vspace{-6mm}

where $\mathbf{W}_{*}$ and $\mathbf{b_g}$ are trainable parameters, and $\sigma$ is a sigmoid nonlinear transformation. The same operation is conducted on sentence b, thus having the outputs $\widehat{\mathbf{H}}_{a}$ and $\widehat{\mathbf{H}}_{b}$. By doing this, model can flexibly interpolate the aligned information to the original representations through setting the gate, especially when multiple interaction blocks are applied.
% Especially when multiple interaction blocks are applied, model can decide how much aligned information in different levels to be propagated to the following layers.
Also, this is similar as a skip connection which can prevent the additional model complexity coming from stacked interactions and reduce the training difficulty. We discuss how gate operation enables deeper structures with stacked interaction blocks in Section \ref{ablation}.
% Also, in the case of multiple interaction blocks are stacked, the model will learn how much new information from different levels of interactions to integrate to the original representations by setting the gates.


\subsection{Aggregation Layer}\label{Aggregation Layer}
% We apply an aggregation layer to produce the final representations for each sentence on the top of interaction blocks. A convolutional neural network (with padding) is used to obtain high-level semantic representations. 
We apply a convolutional neural network (with padding) to obtain high-level semantic representations for each sentence on the top of interaction blocks. 
% Formally, given the outputs of the last interaction blocks: $\mathbf{H}^k_a=[\mathbf{h}^k_{a_1}, ..., \mathbf{h}^k_{a_i}, ..., \mathbf{h}^k_{a_m}]$ and $\mathbf{H}^k_b=[\mathbf{h}^k_{b_1}, ..., \mathbf{h}^k_{b_i}, ..., \mathbf{h}^k_{b_m}]$, we get the aggregated representations:
Formally, given the outputs of the interaction blocks, we get the aggregated representations:

\vspace{-5mm}
{\fontsize{10}{11}\selectfont
% \setlength{\abovedisplayskip}{2pt}
% \setlength{\belowdisplayskip}{2pt}
\begin{align}
&\mathbf{V}_a = CNN(\mathbf{U}_a) \\
&\mathbf{V}_b = CNN(\mathbf{U}_b)
\end{align}
\vspace{-6mm}
}

where $\mathbf{U}_a$, $\mathbf{U}_b$ are the outputs of the last interaction block, and $\mathbf{V}_a$, $\mathbf{V}_b$ are the aggregated sentence representations and will be used as the inputs for the prediction layer.


\subsection{Prediction Layer}\label{Prediction Layer}
To get the vector representations of each sequence, we apply mean and max pooling on $\mathbf{V}_a$ and $\mathbf{V}_b$~\cite{liang-etal-2019-asynchronous} to produce both global and salient semantic features:
% The final combined feature vector is obtained by the concatenation of different operations as~\cite{liang-etal-2019-asynchronous}:

\vspace{-5mm}
{\fontsize{10}{11}\selectfont
% \setlength{\abovedisplayskip}{2pt}
% \setlength{\belowdisplayskip}{2pt}
\begin{align}
&\mathbf{V}^{mean}_{a} = \frac{1}{m}{\sum_{i=1}^{m}{\mathbf{v}_{a_i}}}, \mathbf{V}^{max}_{a} = \max_{i=1}^{m}{\mathbf{v}_{a_i}} \\
&\mathbf{V}^{mean}_{b} = \frac{1}{n}{\sum_{j=1}^{n}{\mathbf{v}_{b_j}}}, \mathbf{V}^{max}_{b} = \max_{j=1}^{n}{\mathbf{v}_{b_j}} \\
& \mathbf{V}^{\prime}_{a}=[\mathbf{V}^{mean}_{a};\mathbf{V}^{max}_{a}], \mathbf{V}^{\prime}_{b}=[\mathbf{V}^{mean}_{b};\mathbf{V}^{max}_{b}] 
\end{align}
\vspace{-5mm}
}

\noindent Then we combined $\mathbf{V}^{\prime}_{a}$ and $\mathbf{V}^{\prime}_{b}$ to produce the final feature vector by concatenating the different operations:

\vspace{-5mm}
{\fontsize{10}{11}\selectfont
% \setlength{\abovedisplayskip}{2pt}
% \setlength{\belowdisplayskip}{2pt}
\begin{align}
&\mathbf{V}=[\mathbf{V}^{\prime}_{a};\mathbf{V}^{\prime}_{b};
\mathbf{V}^{\prime}_{a} - \mathbf{V}^{\prime}_{b}; \mathbf{V}^{\prime}_{a} \odot \mathbf{V}^{\prime}_{b}]
\end{align}
\vspace{-6mm}
}

\noindent Finally the prediction layer takes as input the feature vector  $\mathbf{V}$, and passes it to a multi-layer feed-forward neural network (MLP) to calcuate the final target. Softmax is applied onto the final layer to get the probability distributions for each class. 


==> related.tex <==



The task of natural language inference or textual entailment recognition has a long history in natural language processing. 
Early explorations relied on hand-crafted features and traditional NLP pipeline approaches \cite{maccartney-manning-2008-modeling,heilman2010tree}. 

Recent deep neural network models have shown promising results in this area with the availability of large-scale datasets~\cite{bowman-etal-2015-large,williams-etal-2018-broad,khot2018scitail,wang2020multi,peng2020enhanced}. 
In this regard, the conceptually simpler sentence encoding approach aims to first learn good sentence representations and then makes a prediction based on the combination of sentence representations~\cite{mou-etal-2016-natural,conneau-etal-2017-supervised,yin-schutze-2015-convolutional}. However, such models neglect fine-granular sentence interaction information. The sentence interaction approach instead adopts an attention mechanism to match the two sequences and subsequently aggregates the aligned features to obtain high-level representations and predictions. \newcite{wang-jiang-2016-learning} use a match-LSTM to perform word-by-word matching of the hypothesis with the premise. \newcite{parikh-etal-2016-decomposable} employ a decomposable attention method that computes word pair interactions and soft alignments. BiMPM~\cite{wang2017bilateral} matches the two encoded sentences in two directions with a multi-perspective matching operation, and aggregates the matching results with another Bi-LSTM. Nonetheless, these architectures remain relatively shallow and have trouble capturing more complex semantic relations.

The DIIN  model~\cite{gong2017natural} solves text matching tasks by extracting semantic features from an interaction space, and adopts a DenseNet as a convolutional feature extractor. \newcite{chen-etal-2018-neural-natural} propose a knowledge-based inference model with enrichment of external knowledge in calculating coattention, collecting local inferences, and composing the inference. RE2~\cite{yang-etal-2019-simple} has shown strong performance and fast inference speed by focusing on three forms of interaction features.
\newcite{duan2018attention} leverages a deep structure with joint cross-attention and self-attention. However, context features are not well considered when computing cross-sentence attention in the aforementioned systems.

Recently pre-trained language models have been in the center of attention, trained on large-scale corpora and subsequently fine-tuned for various downstream tasks~\cite{devlin-etal-2019-bert,liu2019roberta,sun2019ernie}. Despite achieving promising performance on many natural language understanding problems, these architectures usually have a large parameter size and are hard to be deployed in many applications with the requirement of inference speed. 
Also, they only adopt self-attention over the concatenation of two sequences, and it is unclear whether inter-alignment can be effectively learned.
Our work adopts an interaction-based structure to model sentence relationships and achieves comparative results while maintaining less computational complexity.

Multi-hop attention mechanisms have yielded improvements on machine comprehension~\cite{gong-bowman-2018-ruminating,wang-etal-2018-multi} and implicit argument prediction~\cite{cheng2019implicit}. Different from the above methods, our two-hop attention mechanism consists of self-attention and cross-attention, which strengthens the model's capacity to capture salient contextual information for a proper alignment. A gate fusion layer is adopted to flexibly integrate the aligned representations, and multiple interaction blocks are stacked to conduct alignments at multiple scales.

